Uncovering Latent Reasoning Strategies in Language Models

A language model $p_\theta(y \mid x)$ trained on reasoning tasks learns to solve problems via multiple distinct strategies, yet these strategies are implicit and entangled within the model's response distribution. We study the problem of decomposing the response distribution of a given pretrained language model into a structured, strategy-conditioned representation. Specifically, we learn a latent-variable factorization $p_\theta(y \mid x) \leadsto (r_\phi(z \mid x), g_\phi(y \mid x,z))$, where a router $r$ maps each input to a distribution over latent strategies $z$ and a generator $g$ produces the response conditioned on that strategy. A key challenge is that the generator, initialized from the base model, already represents $p_\theta(y \mid x)$ without using $z$. Standard variational inference therefore gives the model no incentive to route information through $z$ and can yield a severe form of posterior collapse. To address this, we propose a variational objective that measures fractional information gain relative to the base model's response loss and concentrates reconstruction pressure on tokens with high base model surprisal, encouraging $z$ to encode strategy-relevant response variation. We introduce a benchmark of multi-strategy algorithmic tasks and show that this objective recovers latent codes aligned with distinct reference strategies while preserving the base model's response distribution.

==> figstyle.tex <==
%% Shared TikZ figure style.
%%
%% Keep this file focused on reusable visual language: paper colors,
%% semantic aliases, and small TikZ styles. Figure-specific geometry should
%% stay in the individual figure files.

%% Paul Tol vibrant qualitative palette:
%% https://sronpersonalpages.nl/~pault/
\providecolor{figTolBlue}{HTML}{0077BB}
\providecolor{figTolCyan}{HTML}{33BBEE}
\providecolor{figTolTeal}{HTML}{009988}
\providecolor{figTolOrange}{HTML}{EE7733}
\providecolor{figTolMagenta}{HTML}{EE3377}
\providecolor{figTolRed}{HTML}{CC3311}
\providecolor{figTolGray}{HTML}{BBBBBB}

%% Neutral structure colors.
\colorlet{figInk}{black!82}
\colorlet{figMuted}{black!55}
\colorlet{figLine}{black!60}
\colorlet{figPanelFill}{black!4}
\colorlet{figInactive}{black!42}
\colorlet{figInactiveFill}{black!5}

%% Semantic figure roles.
%% Router / strategy uses magenta (high-chroma "pop" hue) so the latent /
%% branching content reads as the visual protagonist. Posterior uses
%% orange under the muted treatment so training-only inference recedes.
\colorlet{figRouter}{figTolMagenta}
\colorlet{figRouterText}{figTolMagenta!85!black}
\colorlet{figRouterFill}{figTolMagenta!12}
\colorlet{figRouterLightFill}{figTolMagenta!5}

\colorlet{figGenerator}{figTolBlue}
\colorlet{figGeneratorText}{figTolBlue!82!black}
\colorlet{figGeneratorFill}{figTolBlue!7}
\colorlet{figGeneratorPanelFill}{figTolBlue!8}

\colorlet{figPosterior}{figTolOrange}
\colorlet{figPosteriorText}{figTolOrange!85!black}
\colorlet{figPosteriorBorder}{figTolOrange}
\colorlet{figPosteriorFill}{figTolOrange!14}
\colorlet{figPosteriorBell}{figTolOrange!24}
\colorlet{figPosteriorPanelFill}{figTolOrange!7}

\colorlet{figBranch}{figRouter}
\colorlet{figBranchText}{figRouterText}
\colorlet{figBranchFill}{figRouterFill}
\colorlet{figDeterministic}{figGenerator}
\colorlet{figDeterministicText}{figGeneratorText}
\colorlet{figDeterministicFill}{figGeneratorFill}
\colorlet{figBaseline}{figTolGray}

\tikzset{
  figToken/.style = {
    draw=figLine, rounded corners=1.5pt, fill=white,
    font=\scriptsize, inner sep=2pt
  },
  figLatentBox/.style = {
    draw=figRouterText, thick, rounded corners=1.5pt,
    fill=figRouterFill, font=\scriptsize, inner sep=2pt
  },
  figHiddenBox/.style = {
    draw=figGenerator!55, rounded corners=1.5pt,
    fill=figGeneratorFill, font=\scriptsize, inner sep=2pt
  },
  figRouterHead/.style = {
    draw=figRouterText, thick, rounded corners=1.5pt,
    fill=figRouterLightFill, font=\scriptsize, inner sep=2pt
  },
  figGeneratorBlock/.style = {
    draw=figGenerator!55, rounded corners=4pt,
    fill=figGeneratorPanelFill, align=center
  },
  figPosteriorToken/.style = {
    figToken, draw=figPosteriorBorder, fill=figPosteriorFill,
    text=figPosteriorText
  },
  figPosteriorHidden/.style = {
    figHiddenBox, draw=figPosteriorBorder, fill=figPosteriorFill,
    text=figPosteriorText
  },
  figPosteriorHead/.style = {
    figRouterHead, draw=figPosteriorBorder, fill=figPosteriorFill,
    text=figPosteriorText
  },
  figPosteriorBox/.style = {
    draw=figPosteriorBorder, rounded corners=3pt,
    fill=figPosteriorFill, dashed, text=figPosteriorText
  },
  figPosteriorPanel/.style = {
    fill=figPosteriorPanelFill, draw=figPosteriorBorder,
    dashed, rounded corners=4pt
  },
  figArrow/.style = {-Stealth, semithick, figInk},
  figMutedArrow/.style = {-Stealth, dashed, semithick, figMuted},
  figSampleArrow/.style = {-Stealth, dashed, thick, figRouterText},
  figPosteriorArrow/.style = {-Stealth, dashed, semithick, figPosteriorBorder},
  figPosteriorTrainArrow/.style = {-Stealth, dashed, thick, figPosteriorBorder},
  figRootNode/.style = {
    figToken, minimum width=7mm, minimum height=4.5mm
  },
  figBranchNode/.style = {
    draw=figBranchText, thick, fill=figBranchFill,
    circle, minimum size=4.5mm, inner sep=0pt
  },
  figDeterministicNode/.style = {
    draw=figDeterministic!55, fill=figDeterministicFill,
    circle, minimum size=4mm, inner sep=0pt
  },
  figInactiveNode/.style = {
    draw=figInactive, fill=figInactiveFill,
    circle, minimum size=2.5mm, inner sep=0pt
  },
  figPathEdge/.style = {-Stealth, semithick, figBranchText},
  figInactiveEdge/.style = {dashed, semithick, figInactive},
  figSmallBarGenerator/.style = {
    fill=figGenerator!50, draw=figGenerator!75, line width=0.2pt
  },
  figSmallBarBranch/.style = {
    fill=figBranch!55, draw=figBranchText, line width=0.25pt
  },
  figSmallBarDeterministic/.style = {
    fill=figDeterministic!35, draw=figDeterministic!70, line width=0.25pt
  },
  figAxis/.style = {figLine, line width=0.3pt},
}


==> shared/figures/token-weighting/strip.tex <==
%% Panel — Linearized token strip with per-token b_t and w_t bars.
%%
%% Standalone TikZ picture; see ../shared/figures/token-weighting/figure.tex for the
%% composed (side-by-side) figure. The strip can also be input directly
%% inside a custom minipage / wrapfigure for half-width layouts.

\begin{tikzpicture}[
  font=\footnotesize,
  >=Stealth,
  tokbox/.style = {
    figToken,
    minimum width=7mm, minimum height=4.0mm
  },
]

  %% ---- Coordinate scaffolding (panel-local; starts at x ≈ 0) ----------
  \def\sXa{0.40}
  \def\sXb{1.25}
  \def\sXc{2.10}
  \def\sXd{2.95}
  \def\sXe{3.80}
  \def\sXf{4.65}

  \def\toY{0.10}     % token row (vertical center)
  \def\bBase{0.45}   % b_t bar baseline (bars grow upward)
  \def\wBase{-0.25}  % w_t bar baseline (bars hang downward)

  %% ---- b_t bars above the tokens -------------------------------------
  %% Branch positions tall; deterministic positions short.
  \fill[figSmallBarBranch]
    (\sXa-0.18, \bBase) rectangle (\sXa+0.18, \bBase+0.95);
  \fill[figSmallBarDeterministic]
    (\sXb-0.18, \bBase) rectangle (\sXb+0.18, \bBase+0.14);
  \fill[figSmallBarBranch]
    (\sXc-0.18, \bBase) rectangle (\sXc+0.18, \bBase+0.80);
  \fill[figSmallBarDeterministic]
    (\sXd-0.18, \bBase) rectangle (\sXd+0.18, \bBase+0.11);
  \fill[figSmallBarDeterministic]
    (\sXe-0.18, \bBase) rectangle (\sXe+0.18, \bBase+0.09);
  \fill[figSmallBarDeterministic]
    (\sXf-0.18, \bBase) rectangle (\sXf+0.18, \bBase+0.07);
  \draw[figAxis]
    ({\sXa-0.35}, \bBase) -- ({\sXf+0.35}, \bBase);
  \node[font=\scriptsize, anchor=east]
    at ({\sXa-0.42}, {\bBase+0.50}) {$b_t$};

  %% ---- Tokens --------------------------------------------------------
  \node[tokbox] at (\sXa, \toY) {$y_1$};
  \node[tokbox] at (\sXb, \toY) {$y_2$};
  \node[tokbox] at (\sXc, \toY) {$y_3$};
  \node[tokbox] at (\sXd, \toY) {$y_4$};
  \node[tokbox] at (\sXe, \toY) {$y_5$};
  \node[tokbox] at (\sXf, \toY) {$y_6$};

  %% ---- w_t bars below the tokens (mirror of b_t, normalized) ---------
  %% Heights = b_t / Σ b_s × (vertical budget).
  \fill[figSmallBarBranch]
    (\sXa-0.18, \wBase) rectangle (\sXa+0.18, \wBase-0.55);
  \fill[figSmallBarDeterministic]
    (\sXb-0.18, \wBase) rectangle (\sXb+0.18, \wBase-0.07);
  \fill[figSmallBarBranch]
    (\sXc-0.18, \wBase) rectangle (\sXc+0.18, \wBase-0.46);
  \fill[figSmallBarDeterministic]
    (\sXd-0.18, \wBase) rectangle (\sXd+0.18, \wBase-0.06);
  \fill[figSmallBarDeterministic]
    (\sXe-0.18, \wBase) rectangle (\sXe+0.18, \wBase-0.05);
  \fill[figSmallBarDeterministic]
    (\sXf-0.18, \wBase) rectangle (\sXf+0.18, \wBase-0.04);
  \draw[figAxis]
    ({\sXa-0.35}, \wBase) -- ({\sXf+0.35}, \wBase);
  \node[font=\scriptsize, anchor=east]
    at ({\sXa-0.42}, {\wBase-0.27}) {$w_t$};

\end{tikzpicture}%


==> shared/figures/token-weighting/tree.tex <==
%% Panel — Reasoning-tree fragment with one path highlighted.
%%
%% Standalone TikZ picture (no figure environment, no \resizebox). The
%% caller wraps this in a figure / minipage / wrapfigure as needed; the
%% canonical use is ../shared/figures/token-weighting/figure.tex which composes
%% this panel side-by-side with ../shared/figures/token-weighting/strip.tex.

\begin{tikzpicture}[
  font=\footnotesize,
  >=Stealth,
  %% Local aliases delegate to figstyle.tex; no extra attributes here so
  %% sizes / shapes / colors stay owned by the shared style file.
  rootnode/.style   = {figRootNode},
  branchnode/.style = {figBranchNode},
  detnode/.style    = {figDeterministicNode},
  altnode/.style    = {figInactiveNode},
  pathedge/.style   = {figPathEdge},
  altedge/.style    = {figInactiveEdge},
]

  %% ---- Coordinate scaffolding ----------------------------------------
  \def\rX{0.0}
  \def\pXa{1.05}
  \def\pXb{1.95}
  \def\pXc{2.85}
  \def\pXd{3.75}
  \def\pXe{4.65}
  \def\pXf{5.55}

  \def\trY{1.40}        % path node row
  \def\trYglyph{2.20}   % distribution glyph baseline
  \def\trYaltU{1.85}    % up-fork sibling endpoints
  \def\trYaltD{0.95}    % down-fork sibling endpoints

  %% ---- Root x and chosen path's nodes (alternating branch / det) -----
  \node[rootnode]   (root) at (\rX,  \trY) {$x$};
  \node[branchnode] (n1)   at (\pXa, \trY) {};
  \node[detnode]    (n2)   at (\pXb, \trY) {};
  \node[branchnode] (n3)   at (\pXc, \trY) {};
  \node[detnode]    (n4)   at (\pXd, \trY) {};
  \node[detnode]    (n5)   at (\pXe, \trY) {};
  \node[detnode]    (n6)   at (\pXf, \trY) {};

  \draw[pathedge] (root.east) -- (n1.west);
  \draw[pathedge] (n1.east)   -- (n2.west);
  \draw[pathedge] (n2.east)   -- (n3.west);
  \draw[pathedge] (n3.east)   -- (n4.west);
  \draw[pathedge] (n4.east)   -- (n5.west);
  \draw[pathedge] (n5.east)   -- (n6.west);

  %% ---- Sibling branches at branch nodes (alt strategies, not taken) ---
  \node[altnode] (a1u) at ({\pXa+0.55}, \trYaltU) {};
  \node[altnode] (a1d) at ({\pXa+0.55}, \trYaltD) {};
  \draw[altedge] (n1) -- (a1u);
  \draw[altedge] (n1) -- (a1d);

  \node[altnode] (a3u) at ({\pXc+0.55}, \trYaltU) {};
  \node[altnode] (a3d) at ({\pXc+0.55}, \trYaltD) {};
  \draw[altedge] (n3) -- (a3u);
  \draw[altedge] (n3) -- (a3d);

  %% ---- Token labels under path nodes ---------------------------------
  \node[font=\scriptsize, anchor=north] at (n1.south) {$y_1$};
  \node[font=\scriptsize, anchor=north] at (n2.south) {$y_2$};
  \node[font=\scriptsize, anchor=north] at (n3.south) {$y_3$};
  \node[font=\scriptsize, anchor=north] at (n4.south) {$y_4$};
  \node[font=\scriptsize, anchor=north] at (n5.south) {$y_5$};
  \node[font=\scriptsize, anchor=north] at (n6.south) {$y_6$};

  %% ---- Distribution glyphs above each path node ----------------------
  %% Generic 5-bar histogram glyph.
  %%   #1 = x-center, #2 = y-baseline, #3 = bar fill style key
  %%       (figSmallBarBranch / figSmallBarDeterministic / figSmallBarGenerator),
  %%   #4..#8 = bar heights for positions 1..5.
  %% Heights ≤ ~0.45 to fit the panel's headroom.
  \providecommand{\histGlyph}[8]{%
    \begin{scope}[shift={(#1, #2)}]
      \fill[#3] (-0.30, 0) rectangle (-0.18, #4);
      \fill[#3] (-0.18, 0) rectangle (-0.06, #5);
      \fill[#3] (-0.06, 0) rectangle ( 0.06, #6);
      \fill[#3] ( 0.06, 0) rectangle ( 0.18, #7);
      \fill[#3] ( 0.18, 0) rectangle ( 0.30, #8);
      \draw[figAxis] (-0.32, 0) -- (0.32, 0);
    \end{scope}
  }

  %% Branch glyphs are multi-modal but distinct from each other.
  %% Det glyphs are sharply peaked, each on a different token, so the
  %% determined-continuation regime does not look like a single repeated
  %% distribution copy-pasted across positions.

  %% Branch (y_1): two strong modes at positions 2 & 4.
  \histGlyph{\pXa}{\trYglyph}{figSmallBarBranch}{0.10}{0.34}{0.12}{0.30}{0.16}
  %% Det (y_2): sharply peaked at position 1.
  \histGlyph{\pXb}{\trYglyph}{figSmallBarDeterministic}{0.42}{0.06}{0.04}{0.03}{0.05}
  %% Branch (y_3): three asymmetric peaks (different shape from y_1).
  \histGlyph{\pXc}{\trYglyph}{figSmallBarBranch}{0.20}{0.12}{0.32}{0.24}{0.06}
  %% Det (y_4): peaked at position 4.
  \histGlyph{\pXd}{\trYglyph}{figSmallBarDeterministic}{0.04}{0.05}{0.03}{0.40}{0.04}
  %% Det (y_5): peaked at position 2.
  \histGlyph{\pXe}{\trYglyph}{figSmallBarDeterministic}{0.05}{0.38}{0.04}{0.03}{0.05}
  %% Det (y_6): peaked at position 5.
  \histGlyph{\pXf}{\trYglyph}{figSmallBarDeterministic}{0.03}{0.04}{0.05}{0.06}{0.42}

\end{tikzpicture}%

